OpenBox: A Generalized Black-box Optimization Service

Black-box optimization (BBO) has a broad range of applications, including automatic machine learning, engineering, physics, and experimental design. However, it remains a challenge for users to apply BBO methods to their problems at hand with existing software packages, in terms of applicability, performance, and efficiency. In this paper, we build OpenBox, an open-source and general-purpose BBO service with improved usability. The modular design behind OpenBox also facilitates flexible abstraction and optimization of basic BBO components that are common in other existing systems. OpenBox is distributed, fault-tolerant, and scalable. To improve efficiency, OpenBox further utilizes "algorithm agnostic" parallelization and transfer learning. Our experimental results demonstrate the effectiveness and efficiency of OpenBox compared to existing systems.

==> backup.tex <==
\begin{abstract}
Black-box optimization has a broad range of applications, including automatic machine learning, engineering, physics, and experimental design.
However, it is not easy for users to apply black-box optimization methods to their problems using the existing software packages in terms of applicability, performance and efficiency. 
In this paper, we adopt the ``black-box optimization as a service'' paradigm for ease of use, and build a general system named \sys, which is the first open-source service for black-box optimization.
\sys's modular design facilitates flexible abstraction and optimization of basic elements in black-box optimization.
We further implement it as a distributed, fault-tolerant and scalable service.  
To improve efficiency, \sys provides
the algorithm-agnostic parallelization and transfer-learning framework.
In experiments, we demonstrate the effectiveness and efficiency of \sys relative to the existing packages.

% Data mining applications are typically associated with
% systems involving massive complex software systems, large-scale heterogeneous computing and storage architectures. 
% The construction of such systems involves many design choices. 
% To find the optimal design configuration, it becomes easier to experiment with than to understand.
% Therefore, black-box optimization has become increasingly important as these systems have become more complex.
% In this paper, we introduce \sys, an efficient service for black-box optimization, which is the first general-purpose service that provides the powerful functionality of solving the generalized black-box problems. 

% \begin{itemize}
%     \item Bayesian optimization provides sample-efficient global optimization for a broad range of applications, including automatic machine learning, engineering, physics, and experimental design.
%     \item Bayesian optimization (BO), an established methodology for sample-efficient sequential optimization, has been proposed as an effective solution to such problems, and has been applied successfully to tasks ranging from hyperparameter optimization, robotic control, chemical design, and tuning and policy search for internet-scale software systems. 
% \end{itemize}

\end{abstract}
